Use of convexity in contour detection

In this paper, we formulate a simple algorithm that detects contours around a region of interest in an image. After an initial smoothing, the method is based on viewing an image as a topographic surface and finding convex and/or concave regions using simple calculus-based testing. The algorithm can achieve multi-scale contour detection by altering the initial smoothing. We show that the method has promise by comparing results on several images with the watershed transform performed on the gradient images.

==> outtakes.tex <==
\cite{beucher1992morphological} - contains same bubble images!! blobs in radioactive material!! also mentions overlapping structures.

\cite{meyer1990morphological} - has a section on undersegmentation.

\cite{roerdink2000watershed} - discusses the plateau problem and other pitfalls. talks about different definitions, algorithms - immersion, topographical distance, 

The original paper actually just uses watersheds for contour detection, not segmentation, \cite{beucher1979use}. In this application, contours are defined as the watershed of the variation function (gradient modulus) of the image considered as a relief surface. Why? it gives a rigorous mathematical definition of the objects under study, it furnishes a mode of operation, the result is visually satisfactory. In this paper two applications are considered: bubble detection in a radiographic plate, and facet detection in fractures in steel. In 1979, the methods for detecting contours were thresholding the gradient and image segmentation on the pixel values. No threshold is used in watersheds. Every object in a picture corresponds to the minimum of the grey variation function.

The continuous approach is thoroughly covered in \cite{najman1994watershed}

Consider a drop of water which falls on the surface. The water flows down to a minimum and stops. The set of all points of the surface which the drops of water reaching this minimum can come from can be associated with each minimum. Such a set of points is a catchment basin of the surface. Several catchment basins can overlap. Their common points form the watersheds.

%There are several advantages to this technique. After an initial smoothing, the method always forms closed contours, typically does not oversegment given initial smoothing, and is extremely simple heuristically and in the code.  Altering the size of the smoothing kernal enables us to different sized features of the image. Finally, the idea and the code scales easily to three dimensional image stacks, and in theory higher dimensional problems.

%The watershed transform is frequently applied to gradient images in order to identify catchment basins in images by outlining them. Additionally, there are various pre- and post-processing techniques applied to the watershed transform to identify these regions.

Here we take the approach of pre-processing in order to avoid oversegmentation. Note that the option of merging an oversegmentation based on a similarity criterion is still available for this method.

\cite{meyer1994topographic} - The watershed line is the key tool from mathematical morphology for segmenting images. Mainly used on gradient images, detects catchment basins of all minima. The image is considered as a topographical relief. This relief is flooded; the sources are placed at the regional minima. The level of the flood is uniform over the relief and increases with uniform speed. The moment that the floods filling two distinct catchment basins start to merge, a dam is erected in order to prevent mixing of the floods. The union of all dams constitutes the watershed line.

Shape operator is the Hessian, I think. The principal curvatures are the eigenvalues of the shape operator, the principal curvature directions are its eigenvectors, the Gauss curvature is its determinant, and the mean curvature is half its trace.

The watershed transformation has long been used to detect contours in images, \cite{beucher1979use}. Originally, the watershed transform was based on the concept of viewing an image as a topographic surface where the height is given by the intensity value at each pixel. The surface is flooded from below, forming catchment basins. As the water rises, if two catchment basins are to be joined into one, a dam is placed. The dam points make up the watershed line. Later, the watershed transform was formulated using the concepts of topographic distance and steepest descent, \cite{meyer1994topographic}, and later still the concepts of graph connectedness and the optimal spanning forest, \cite{roerdink2000watershed}. 

